CloudFixer: Test-Time Adaptation for 3D Point Clouds via Diffusion-Guided Geometric Transformation

3D point clouds captured from real-world sensors frequently encompass noisy points due to various obstacles, such as occlusion, limited resolution, and variations in scale. These challenges hinder the deployment of pre-trained point cloud recognition models trained on clean point clouds, leading to significant performance degradation. While test-time adaptation (TTA) strategies have shown promising results on this issue in the 2D domain, their application to 3D point clouds remains under-explored. Among TTA methods, an input adaptation approach, which directly converts test instances to the source domain using a pre-trained diffusion model, has been proposed in the 2D domain. Despite its robust TTA performance in practical situations, naively adopting this into the 3D domain may be suboptimal due to the neglect of inherent properties of point clouds, and its prohibitive computational cost. Motivated by these limitations, we propose CloudFixer, a test-time input adaptation method tailored for 3D point clouds, employing a pre-trained diffusion model. Specifically, CloudFixer optimizes geometric transformation parameters with carefully designed objectives that leverage the geometric properties of point clouds. We also substantially improve computational efficiency by avoiding backpropagation through the diffusion model and a prohibitive generation process. Furthermore, we propose an online model adaptation strategy by aligning the original model prediction with that of the adapted input. Extensive experiments showcase the superiority of CloudFixer over various TTA baselines, excelling in handling common corruptions and natural distribution shifts across diverse real-world scenarios. Our code is available at https://github.com/shimazing/CloudFixer

==> tables/ablation_chamfer.tex <==
\begin{table}[ht]
\centering
\caption{Ablation study on CloudFixer investigating the influence of Chamfer distance. In this analysis, we assess the effect of employing Chamfer distance, designed to accommodate the unordered nature of 3D point clouds, as opposed to squared $\ell_2$ distance. The hyperparameters for this experiment are configured with a learning rate of $2 \cdot 10^{-1}$, lr warmup of 0, and $t_{max}$ set to $0.22T$.}
% \vspace{-.1in}
%\resizebox{\columnwidth}{!}{
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\label{tab:ablation_chamfer}
\begin{tabular}{l|ccc}
    \Xhline{3\arrayrulewidth}

    \bf Setting & \bf LD & \bf GAU & \bf RBF \\ \Xhline{2\arrayrulewidth}

    \bf Unadapted & 25.81 & 84.08 & 84.24 \\\hdashline
    
    \bf Squared $\ell_2$ Dist. & 33.35 & 88.89 & 84.31 \\
    
    \bf Chamfer Dist. & \bf 37.31 & \bf 89.66 & \bf 85.57  \\
    
    \Xhline{3\arrayrulewidth}
\end{tabular}%}
% \vspace{-.2in}
\end{table}

==> tables/bsz_1_full.tex <==
\begin{table*}[t]
    \centering
    \caption{Experimental results in a limited batch size scenario (batch size of 1) for each corruption type on ModelNet40-C, measured as accuracy. The averaged accuracy across all corruption types is reported in the \emph{4th} column of \Cref{table:scenario}.}
    \label{table:bsz_1_full}
    % \vspace{-.1in}
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|ccccc|c}
    \Xhline{3\arrayrulewidth}

    \multirow{2}{*}{\bf Method} & \multicolumn{5}{c|}{\bf Density Corruptions} &  \multicolumn{5}{c|}{\bf Noise Corruptions} &  \multicolumn{5}{c|}{\bf Transformation Corruptions} & \multirow{2}{*}{\bf Avg.} \\ \cline{2-16}
    
    & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \Xhline{2\arrayrulewidth}

    \bf Unadapted & 40.40 & 25.81 & \bf 90.32 & \bf 87.36 & 88.29 & 86.02 & 84.08 & 87.24 & 81.60 & 89.10 & 66.37 & \bf 88.45 & \bf 86.14 & 84.24 & 86.14 & 78.10 \\ \hdashline

    \bf PL & 0.81 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 3.83 \\
    
    \bf TENT & 4.50 & 4.17 & 39.30 & 10.33 & 79.54 & 7.90 & 8.71 & 64.71 & 4.17 & 5.55 & 6.93 & 32.58 & 17.14 & 12.20 & 17.91 & 21.04 \\
    
    \bf SHOT & 0.81 & 0.81 & 4.09 & 4.09 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.09 & 3.53 & 4.05 & 4.09 & 4.05 & 4.05 & 3.59 \\
    
    \bf SAR & 28.97 & 19.69 & 11.71 & 79.29 & 16.53 & 71.31 & 66.09 & 75.45 & 58.27 & 51.99 & 62.88 & 13.41 & 76.26 & 72.85 & 74.27 & 51.93 \\
    
    \bf DUA & 32.78 & 23.06 & 82.01 & 82.05 & 81.36 & 74.07 & 70.95 & 76.62 & 61.51 & 58.63 & 68.15 & 82.17 & 77.76 & 75.36 & 76.94 & 68.23 \\ \hline
    
    \bf LAME & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 & 4.05 \\

    \bf MEMO & 34.81 & 26.30 & 84.40 & 83.79 & 83.35 & 73.82 & 70.91 & 77.31 & 57.54 & 57.17 & 71.11 & 85.33 & 80.35 & 77.04 & 78.44 & 69.44 \\ \hline
    
     \bf CloudFixer & \bf 42.87 & \bf 41.28 & 89.38 & 86.87 & \bf 88.37 & \bf 89.71 & \bf 89.87 & \bf 90.23 & \bf 85.98 & \bf 90.31 & \bf 80.75 & 87.23 & 85.57 & \bf 86.12 & \bf 86.91 & \bf 81.43 \\

    \Xhline{3\arrayrulewidth}
    
    \end{tabular}}
\end{table*}

==> tables/bsz_8_full.tex <==
\begin{table*}[t]
    \centering
    \caption{Experimental results in a limited batch size scenario (batch size of 8) for each corruption type on ModelNet40-C, measured as accuracy. The averaged accuracy across all corruption types is reported in the \emph{5th} column of \Cref{table:scenario}.}
    \label{table:bsz_8_full}
    % \vspace{-.1in}
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|ccccc|c}
    \Xhline{3\arrayrulewidth}

    \multirow{2}{*}{\bf Method} & \multicolumn{5}{c|}{\bf Density Corruptions} &  \multicolumn{5}{c|}{\bf Noise Corruptions} &  \multicolumn{5}{c|}{\bf Transformation Corruptions} & \multirow{2}{*}{\bf Avg.} \\ \cline{2-16}
    
    & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \Xhline{2\arrayrulewidth}

    \bf Unadapted & 40.40 & 25.81 & \bf 90.32 & \bf 87.36 & 88.29 & 86.02 & 84.08 & 87.24 & 81.60 & 89.10 & 66.37 & \bf 88.45 & \bf 86.14 & 84.24 & 86.14 & 78.10 \\ \hdashline
    
    \bf PL & 23.01 & 9.28 & 64.06 & 68.96 & 60.66 & 68.48 & 71.68 & 62.12 & 60.05 & 73.91 & 62.56 & 63.25 & 73.18 & 64.38 & 64.34 & 59.33 \\
    
    \bf TENT & 41.41 & 35.70 & 85.98 & 83.83 & 84.72 & 82.86 & 81.65 & 83.79 & 80.31 & 85.37 & 73.54 & 85.01 & 83.06 & 81.85 & 82.90 & 76.80 \\
    
    \bf SHOT & 35.74 & 34.28 & 78.97 & 75.77 & 77.07 & 78.93 & 75.77 & 76.82 & 75.12 & 80.63 & 69.73 & 79.01 & 75.81 & 75.97 & 77.23 & 71.12 \\
    
    \bf SAR & 40.52 & 34.76 & 7.94 & 7.33 & 8.47 & 17.79 & 25.41 & 45.14 & 7.13 & 26.62 & 9.97 & 43.76 & 36.79 & 36.91 & 37.93 & 25.76 \\
    
    \bf DUA & 43.56 & 37.64 & 87.88 & 85.62 & 86.63 & 84.93 & 84.04 & 85.74 & 82.05 & 86.83 & 75.77 & 87.36 & 84.72 & 84.20 & 84.00 & 78.73 \\ \hline
    
    \bf LAME & 38.78 & 21.39 & 89.79 & 87.20 & 88.21 & 85.53 & 83.14 & 85.90 & 80.79 & 88.70 & 64.38 & 88.09 & 85.74 & 83.31 & 85.37 & 77.09 \\

    \bf MEMO & 34.81 & 26.30 & 84.40 & 83.79 & 83.35 & 73.82 & 70.91 & 77.31 & 57.54 & 57.17 & 71.11 & 85.33 & 80.35 & 77.03 & 78.44 & 69.44 \\ \hline
    
     \bf CloudFixer & \bf 42.87 & \bf 41.28 & 89.38 & 86.87 & \bf 88.37 & \bf 89.71 & \bf 89.87 & \bf 90.23 & \bf 85.98 & \bf 90.31 & \bf 80.75 & 87.23 & 85.57 & \bf 86.12 & \bf 86.91 & \bf 81.43 \\ 

    \Xhline{3\arrayrulewidth}
    
    \end{tabular}}
\end{table*}

==> tables/hparam_selected.tex <==
\begin{table*}[t!]
\centering
\caption{Selected hyperparameters for test-time adaptation methods at each batch size.}
\label{table:tta_hyperparam_selected}
\setlength{\columnsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=\linewidth}
% \vspace{-.1in}
\begin{tabular}{l|c|l}
    \Xhline{3\arrayrulewidth}
    \bf Method & \bf Batch Size & \bf Selected Hyperparameters \\ \Xhline{2\arrayrulewidth}
    
    \multirow{3}{*}{\bf PL} & 1 & learning rate: $10^{-2}$, adaptation steps: $10$ \\
    & 8 & learning rate: $10^{-2}$, adaptation steps: $3$ \\
    & 64 & learning rate: $10^{-2}$, adaptation steps: $1$ \\ \hline

    \multirow{3}{*}{\bf TENT} & 1 & learning rate: $10^{-4}$, adaptation steps: $5$ \\
    & 8 & learning rate: $10^{-4}$, adaptation steps: $3$ \\
    & 64 & learning rate: $10^{-4}$, adaptation steps: $10$ \\ \hline

    \multirow{3}{*}{\bf SHOT} & 1 & learning rate: $10^{-4}$, adaptation steps: $5$, pseudo-labeling loss weight: 0.3 \\
    & 8 & learning rate: $10^{-4}$, adaptation steps: $5$, pseudo-labeling loss weight: 0.3 \\
    & 64 & learning rate: $10^{-4}$, adaptation steps: $5$, pseudo-labeling loss weight: 0 \\ \hline

    \multirow{2}{*}{\bf SAR} & 1, 8 & learning rate: $10^{-3}$, adaptation steps: $3$, entropy threshold: 0.2, epsilon threshold: 0.1 \\
    & 64 & learning rate: $10^{-2}$, adaptation steps: $3$, entropy threshold: 0.2, epsilon threshold: 0.1 \\ \hline

    \multirow{3}{*}{\bf DUA} & 1 & adaptation steps: 3, decay factor: 0.94 \\
    & 8 & adaptation steps: 1, decay factor: 0.94 \\
    & 64 & adaptation steps: 5, decay factor: 0.9 \\ \hline

    \multirow{3}{*}{\bf LAME} & 1 & kernel affinity: rbf, \# of neighbors: $3$, max steps: $100$ \\
    & 8 & kernel affinity: rbf, \# of neighbors: $3$, max steps: $1$ \\
    & 64 & kernel affinity: kNN, \# of neighbors: $1$, max steps: $10$ \\ \hline

    \bf MEMO & 1 & learning rate: $10^{-4}$, adaptation steps: $2$, \# of augmentations: $16$ \\ \hline

    \bf DDA & 1 & guidance weight: $6$, low pass filtering scale: $4$ \\ \hline
    
    \bf CloudFixer & 1 & learning rate:  $2 \cdot 10^{-1}$, lr warmup: $0.2$, $\lambda$: $10$, $t_{max}$: $0.12T$ \\
    
    \Xhline{3\arrayrulewidth}
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/imb_correction.tex <==
\begin{table}[htbp]
\centering
\caption{Corrected results of the class imbalance scenario. For this scenario, we report macro recall-score that average recall along the all classes instead of accuracy.}
% \vspace{0.1in}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.1}
\label{tab:imb_correction}
\begin{tabular}{l|c}
    \Xhline{3\arrayrulewidth}
    
    \textbf{Method} & \textbf{Accuracy} \\ \Xhline{2\arrayrulewidth}
    
    Unadapted & 71.84 \\  \hdashline
    
    PL & \\
    
    Tent &  \\
    
    SHOT &  \\
    
    SAR &  \\
    
    DUA &  \\
    
    LAME &  \\
    
    MEMO &  \\\hline
    
    \textbf{CloudFixer} & \textbf{76.25} \\
    
    \Xhline{3\arrayrulewidth}
\end{tabular}
\end{table}

==> tables/imb_full.tex <==
\begin{table*}[t]
    \centering
    \caption{Experimental results the label distribution shift scenario with a high class imbalance ratio (\emph{imbalance ratio} = 10) for each corruption type on ModelNet40-C, measured as a macro-recall score. The averaged macro-recall score across all corruption types is reported in the \emph{2nd} column of \Cref{table:scenario}.}
    \label{table:imb_full}
    % \vspace{-.1in}
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|ccccc|c}
    \Xhline{3\arrayrulewidth}

    \multirow{2}{*}{\bf Method} & \multicolumn{5}{c|}{\bf Density Corruptions} &  \multicolumn{5}{c|}{\bf Noise Corruptions} &  \multicolumn{5}{c|}{\bf Transformation Corruptions} & \multirow{2}{*}{\bf Avg.} \\ \cline{2-16}

    & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \Xhline{2\arrayrulewidth}
    
    \bf Unadapted & 44.38 & 24.01 & \bf 85.07 & 80.31 & 81.12 & 75.49 & 73.40 & 76.69 & 70.67 & 82.79 & 61.11 & \bf 83.84 & \bf 81.94 & 77.42 & 79.42 & 71.84 \\ \hdashline
    
    \bf PL & 46.46 & 34.38 & 82.85 & 78.78 & 80.38 & 80.13 & 79.38 & 79.61 & 73.84 & 83.61 & 69.77 & 80.86 & 79.72 & 77.42 & 80.44 & 73.84 \\

    \bf TENT & 46.80 & 35.24 & 81.66 & 80.20 & 80.38 & 78.47 & 78.13 & 80.03 & 74.01 & 82.38 & 68.79 & 81.99 & 79.50 & 78.45 & 80.16 & 73.75 \\
    
    \bf SHOT & \bf 48.66 & 41.21 & 83.89 & \bf 81.61 & 80.10 & 79.55 & 80.38 & 80.50 & 78.50 & 83.80 & 74.68 & 83.79 & 81.10 & 78.23 & \bf 81.98 & 75.87 \\
    
    \bf SAR & 30.11 & 35.38 & 79.97 & 76.92 & 78.77 & 73.37 & 71.78 & 77.95 & 71.34 & 78.20 & 58.78 & 79.34 & 76.29 & 74.13 & 77.13 & 69.30 \\
    
    \bf DUA & 48.20 & 38.32 & 82.90 & 81.49 & 81.29 & 79.61 & 78.57 & 81.56 & 74.14 & 82.05 & 70.60 & 83.73 & 80.42 & 78.52 & 81.81 & 74.88 \\ \hline
 
    \bf LAME & 45.15 & 23.17 & 83.71 & 80.98 & 81.46 & 75.69 & 73.19 & 76.27 & 71.30 & 82.01 & 59.72 & 82.35 & 81.43 & 76.73 & 78.90 & 71.47 \\

    \bf MEMO & 35.25 & 22.74 & 77.58 & 76.57 & 74.58 & 62.87 & 58.40 & 64.97 & 46.00 & 46.53 & 60.03 & 79.49 & 73.20 & 68.93 & 70.10 & 61.15 \\ \hline
    
    \bf CloudFixer & 46.59 & \bf 44.69 &  83.78 & 80.86 & \bf 83.26 & \bf 83.06 &\bf 83.01 & \bf 84.62 & \bf 79.99 & \bf 84.99 & \bf 76.75 & 83.04 & 80.60 & \bf 80.98 & 80.50 & \bf 77.11 \\


    \Xhline{3\arrayrulewidth}
    
    \end{tabular}}
\end{table*}

==> tables/mixed_corruption.tex <==
\begin{table}[t]
\centering
\caption{Evaluation on mixed corruption cases.}
\label{tab:mixed_corruption}
% \vspace{-0.05in}
\setlength{\tabcolsep}{4pt} 
\renewcommand{\arraystretch}{1.2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccc|cccc}
\Xhline{2\arrayrulewidth}
    \multirow{2}{*}{\bf Method} & \multicolumn{4}{c|}{\bf Severity 5} &  \multicolumn{4}{c}{\bf Severity 3} \\ \cline{2-9}
     & 4 & 8 & 16 & 32 & 4 & 8 & 16 & 32 \\ \Xhline{2\arrayrulewidth}
    Unadapted &  \multicolumn{4}{c|}{85.25} & \multicolumn{4}{c}{90.07}  \\ \hdashline
    DUA &  79.01 & 83.10 & 84.97 & 85.70 & 84.85 & 86.99 & 88.17 & 88.98 \\
    TENT & 74.80 & 79.78 & 82.50 & 82.86 & 79.29 & 84.56 & 86.02 & 87.72 \\
    SHOT & 74.43 & 79.50 & 82.66 & 82.94 & 79.09 & 84.85 & 86.10 & 85.66 \\
    SAR & 74.19 & 79.50 & 82.94 & 83.91 & 78.81 & 84.60 & 86.83 & 87.48 \\ \hline
    CloudFixer & \multicolumn{4}{c|}{\bf 89.34} & \multicolumn{4}{c}{\bf 91.57} \\    
\Xhline{2\arrayrulewidth}
\end{tabular}}
% \vspace{-0.2in}
\end{table}

==> tables/rotation_ablation.tex <==
\begin{table*}[t]
    \centering
    \caption{Results on ModelNet40-C with 15 corruption types and the severity level 5. We report the performance of online TTA baselines with a batch size of 64. The last row represents the results of applying both CloudFixer input adaptation and SHOT with a batch size of 64, which is the best-performing model adaptation baseline on ModelNet40-C.}
    \label{table:rotation_ablation}
    % \vspace{-.1in}
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cl|ccccc|ccccc|ccccc|c}

    \Xhline{3\arrayrulewidth}

    &\multirow{2}{*}{\bf Method} & \multicolumn{5}{c|}{\bf Density Corruptions} &  \multicolumn{5}{c|}{\bf Noise Corruptions} &  \multicolumn{5}{c|}{\bf Transformation Corruptions} & \multirow{2}{*}{\bf Avg.} \\ \cline{3-17}
    
    % & & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \Xhline{2\arrayrulewidth}
    
    & & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \cline{2-18}

    &\bf Unadapted & 40.40 & 25.81 & \bf 90.32 & 87.36 & 88.29 & 86.02 & 84.08 & 87.24 & 81.60 & 89.10 & 66.37 & 88.45 & 86.14 & 84.24 & 86.14 & 78.10 \\ \cdashline{2-18}
    
    &\bf PL & 46.35 & 38.29 & 89.34 & 87.84 & 88.65 & 87.97 & 87.36 & 88.05 & 86.22 & 90.48 & 80.31 & 89.22 & 87.03 & 88.09 & 87.88 & 81.54 \\
    
    &\bf TENT & 45.66 & 39.47 & 88.82 & 86.63 & 88.05 & 87.44 & 86.26 & 88.25 & 85.33 & 88.70 & 78.53 & 88.70 & 86.26 & 86.14 & 86.83 & 80.74 \\

    &\bf SHOT & \bf 51.99 & 46.43 & 89.95 & \bf 88.74 & \bf 89.06 & 89.71 & 88.57 & 89.02 & 88.49 & \bf 91.41 & 84.48 & \bf 90.56 & 88.37 & 88.70 & 89.14 & 83.64 \\

    \rot{\rlap{~\textbf{Online}}} &\bf SAR & 28.36 & 39.02 & 88.17 & 85.21 & 87.44 & 84.64 & 84.36 & 87.76 & 80.11 & 84.36 & 74.76 & 87.24 & 85.33 & 83.55 & 85.62 & 77.73 \\
    
    &\bf DUA & 47.04 & 40.64 & 89.99 & 88.65 & 89.51 & 88.09 & 87.60 & 88.65 & 84.56 & 89.22 & 80.11 & 89.75 & 87.28 & 86.91 & 87.40 & 81.69 \\ \cline{2-18}

    &\bf LAME & 40.40 & 25.16 & 89.95 & 87.68 & 87.68 & 85.94 & 83.79 & 86.75 & 81.81 & 89.06 & 66.09 & 88.86 & 86.26 & 84.04 & 85.94 & 77.96 \\

    &\bf MEMO & 34.81 & 26.30 & 84.40 & 83.79 & 83.35 & 73.82 & 70.91 & 77.31 & 57.54 & 57.17 & 71.11 & 85.33 & 80.35 & 77.03 & 78.44 & 69.44 \\
    
    \rot{\rlap{\textbf{Episodic}}} &\bf DDA & 42.30 & 38.37 & 88.33 & 83.43 & 88.01 & 89.51 & 89.34 & 89.51 & 86.87 & 85.78 & 64.95 & 83.79 & 83.67 & 85.01 & 86.91 & 79.05 \\ \cline{2-18}

    &\bf CloudFixer & 42.87 & 36.34 & 89.14 & 86.06 & 87.19 & 89.10 & 89.10 & 89.24 & 85.09 & 88.45 & 84.76 & 85.99 & 85.74 & 85.98 & 87.35 & 80.83 \\

    &\bf + Soft Voting & 43.24 & 36.95 & 89.58 & 87.08 & 88.25 & 89.62 & 90.11 & \bf 90.13 & 85.77 & 89.42 & 85.69 & 87.40 & 86.46 & 86.87 & 87.76 & 81.62 \\
     
    \rot{\rlap{~~~\textbf{Ours}}}&\bf + SHOT & 51.87 & \bf 51.05 & 89.01 & 87.76 & 88.16 & \bf 90.27 & \bf 90.35 & 90.03 & \bf 89.87 & 90.64 & \bf 88.81 & 89.30 & \bf 88.85 & \bf 89.38 & \bf 89.66 & \bf 84.33 \\

    \Xhline{3\arrayrulewidth}
    
    \end{tabular}}
% \vspace{-.2in}
\end{table*}

==> tables/scenario.tex <==
\begin{table}[t]
\caption{Experimental results on various realistic test-time scenarios including \textbf{Mixed Corruption}, where each sample randomly has one of the 15 corruption types, \textbf{Class Imb.} with situations where a high class imbalance ratio exists, and \textbf{Temporal Correlation}, in case of temporally correlated non-i.i.d test instances given in class order. We also report the performance under limited batch sizes of 1 (\textbf{Bsz. 1}) and 8 (\textbf{Bsz. 8}).}
\label{table:scenario}
\centering
% \vspace{-.15in}
\resizebox{0.7\linewidth}{!}{
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|ccc|cc}
\Xhline{3\arrayrulewidth}
\bf Method & \makecell{\bf Mixed\\\bf Corruption} & \makecell{\bf Class\\\bf Imb.} & \makecell{\bf Temporal\\ \bf Correlation} & \makecell{\bf Bsz. 1} & \makecell{\bf Bsz. 8} \\
    \Xhline{2\arrayrulewidth}
    Unadapted & 77.67 & 71.77 & 78.10 & 78.10 & 78.10 \\\hdashline

    PL & 78.85 & 73.84 & 21.35 & 3.83 & 59.33 \\
    
    TENT & 76.78 & 73.75 & 22.95 & 21.04 & 76.80 \\
    
    SHOT & 79.74 & 75.87 & 21.91 & 3.59 & 71.12 \\
    
    SAR & 75.36 & 69.30 & 21.36 & 51.93 & 25.76 \\
    
    DUA & 78.89 & 74.88 & 24.60 & 68.23 & 78.73 \\ \hline

    LAME & 77.35 & 71.47 & 79.93 & 4.05 & 77.09 \\

    MEMO & 71.23 & 61.15 & 69.44 & 69.44 & 69.44 \\ \hline
    
    \bf CloudFixer & \bf 81.14 & \bf 77.11 & \bf 81.43 & \bf 81.43 & \bf 81.43 \\
    \Xhline{3\arrayrulewidth}
\end{tabular}}
% \vspace{-.2in}
\end{table}

==> tables/temporally_correlated_full.tex <==
\begin{table*}[t]
    \centering
    \caption{Experimental results in a temporally correlated non-i.i.d test instances, whose classes are given in sequence for each corruption type on ModelNet40-C, measured as accuracy. The averaged accuracy across all corruption types is reported in the \emph{3th} column of \Cref{table:scenario}.}
    \label{table:temporally_correlated_full}
    % \vspace{-.1in}
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|ccccc|c}
    \Xhline{3\arrayrulewidth}

    \multirow{2}{*}{\bf Method} & \multicolumn{5}{c|}{\bf Density Corruptions} &  \multicolumn{5}{c|}{\bf Noise Corruptions} &  \multicolumn{5}{c|}{\bf Transformation Corruptions} & \multirow{2}{*}{\bf Avg.} \\ \cline{2-16}

    & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \Xhline{2\arrayrulewidth}

    \bf Unadapted & 40.40 & 25.81 &  90.32 &  87.36 & 88.29 & 86.02 & 84.08 & 87.24 & 81.60 & 89.10 & 66.37 & 88.45 & 86.14 & 84.24 & 86.14 & 78.10 \\ \hdashline

    \bf PL & 14.95 & 11.67 & 27.55 & 23.91 & 25.57 & 23.22 & 23.10 & 24.88 & 10.21 & 21.23 & 19.04 & 23.91 & 24.64 & 22.89 & 23.42 & 21.35 \\
    
    \bf TENT & 16.61 & 12.88 & 27.39 & 26.94 & 26.82 & 23.74 & 23.46 & 26.58 & 11.10 & 24.64 & 21.47 & 26.99 & 25.65 & 24.96 & 25.08 & 22.95 \\
    
    \bf SHOT & 15.68 & 11.43 & 25.61 & 25.28 & 25.32 & 22.93 & 22.77 & 25.08 & 20.83 & 22.61 & 17.75 & 23.99 & 23.78 & 22.61 & 23.01 & 21.91 \\
    
    \bf SAR & 14.51 & 12.44 & 24.92 & 25.77 & 26.26 & 21.11 & 20.50 & 17.83 & 11.87 & 21.07 & 21.23 & 26.94 & 25.81 & 24.68 & 25.49 & 21.36 \\
    
    \bf DUA & 17.30 & 14.06 & 29.34 & 27.88 & 28.04 & 27.31 & 25.65 & 28.08 & 12.76 & 26.18 & 23.14 & 28.93 & 27.03 & 26.38 & 26.90 & 24.60 \\ \hline
    
    \bf LAME & 41.65 & 26.34 & \bf 92.02 & \bf 89.30 & 90.72 & 87.76 & 85.70 & 89.38 & 83.35 & \bf 91.13 & 67.95 & \bf 90.40 & \bf 87.97 & \bf 86.91 & \bf 88.41 & 79.93 \\

    \bf MEMO & 35.09 & 26.22 & 84.12 & 83.75 & 83.27 & 74.23 & 71.39 & 77.43 & 58.02 & 56.20 & 70.58 & 85.25 & 79.54 & 77.07 & 79.01 & 69.41 \\ \hline
    
    \bf CloudFixer & \bf 42.87 & \bf 41.28 & 89.38 & 86.87 & \bf 88.37 & \bf 89.71 & \bf 89.87 & \bf 90.23 & \bf 85.98 &  90.31 & \bf 80.75 & 87.23 & 85.57 & 86.12 & 86.91 & \bf 81.43 \\

    \Xhline{3\arrayrulewidth}
    
    \end{tabular}}
\end{table*}

==> tables/tuned_modelnet40.tex <==
\begin{table*}[htbp]
\centering
\caption{Updated experimental results on ModelNet40-C after optimizing hyperparameters of CloudFixer in the same ways of baselines. ModelNet40-C has 15 corruption types and severity level 5. We report the performance of online TTA baselines with a batch size of 64, measured as accuracy. The last row represents the results of applying both CloudFixer input adaptation and SHOT with a batch size of 64, which is the best-performing model adaptation baseline on ModelNet40-C.}
\label{table:modelnet40c_tuned}
   \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cl|ccccc|ccccc|ccccc|c}
    \Xhline{3\arrayrulewidth}

    &\multirow{2}{*}{\bf Method} & \multicolumn{5}{c|}{\bf Density Corruptions} &  \multicolumn{5}{c|}{\bf Noise Corruptions} &  \multicolumn{5}{c|}{\bf Transformation Corruptions} & \multirow{2}{*}{\bf Avg.} \\ \cline{3-17}
    
    & & \bf OC & \bf LD & \bf DI & \bf DD & \bf CO & \bf UNI & \bf GAU & \bf IP & \bf US & \bf BG & \bf ROT & \bf SH & \bf FFD & \bf RBF & \bf IR & \\ \Xhline{2\arrayrulewidth}

    & \bf Unadapted & 40.40 & 25.81 & \bf 90.32 & 87.36 & 88.29 & 86.02 & 84.08 & 87.24 & 81.60 & 89.10 & 66.37 & 88.45 & 86.14 & 84.24 & 86.14 & 78.10 \\\cdashline{2-18}

    &\bf PL & 46.35 & 38.29 & 89.34 & 87.84 & 88.65 & 87.97 & 87.36 & 88.05 & 86.22 & 90.48 & 80.31 & 89.22 & 87.03 & 88.09 & 87.88 & 81.54 \\
    
    &\bf TENT & 45.66 & 39.47 & 88.82 & 86.63 & 88.05 & 87.44 & 86.26 & 88.25 & 85.33 & 88.70 & 78.53 & 88.70 & 86.26 & 86.14 & 86.83 & 80.74 \\
    
    &\bf SHOT & 51.99 & 46.43 & 89.95 & \bf 88.74 & 89.06 & 89.71 & 88.57 & 89.02 & 88.49 & \bf 91.41 & 84.48 & \bf 90.56 & 88.37 & 88.70 & 89.14 & 83.64 \\
    \rot{\rlap{~\textbf{Online}}} &\bf SAR & 28.36 & 39.02 & 88.17 & 85.21 & 87.44 & 84.64 & 84.36 & 87.76 & 80.11 & 84.36 & 74.76 & 87.24 & 85.33 & 83.55 & 85.62 & 77.73 \\
    
    &\bf DUA & 47.04 & 40.64 & 89.99 & 88.65 & 89.51 & 88.09 & 87.60 & 88.65 & 84.56 & 89.22 & 80.11 & 89.75 & 87.28 & 86.91 & 87.40 & 81.69 \\ \cline{2-18}
    
    &\bf LAME & 40.40 & 25.16 & 89.95 & 87.68 & 87.68 & 85.94 & 83.79 & 86.75 & 81.81 & 89.06 & 66.09 & 88.86 & 86.26 & 84.04 & 85.94 & 77.96 \\
    
    &\bf MEMO & 34.81 & 26.30 & 84.40 & 83.79 & 83.35 & 73.82 & 70.91 & 77.31 & 57.54 & 57.17 & 71.11 & 85.33 & 80.35 & 77.03 & 78.44 & 69.44 \\
    
    \rot{\rlap{\textbf{Episodic}}}  &\bf DDA & 42.30 & 38.37 & 88.33 & 83.43 & 88.01 & 89.51 & 89.34 & 89.51 & 86.87 & 85.78 & 64.95 & 83.79 & 83.67 & 85.01 & 86.91 & 79.05 \\ \cline{2-18}
    
    & \bf CloudFixer & 42.87 & 41.28 & 89.38 & 86.87 & 88.37 & 89.71 & 89.87 & 90.23 & 85.98 & 90.31 & 80.75 & 87.23 & 85.57 & 86.12 & 86.91 & 81.43 \\
    
    &\bf + Soft Voting & 43.11 & 42.46 & 89.58 & 86.99 & 89.18 & 90.07 & 90.56 & \bf 90.96 & 86.30 &  91.07 & 82.45 & 87.76 & 85.94 & 86.22 & 87.76 & 82.03 \\
    
    \rot{\rlap{~~~\textbf{Ours}}} &\bf + SHOT & \bf 53.48 & \bf 52.67 & 89.71 & 88.12 & \bf 89.71 & \bf 91.17 & \bf 91.13 & 90.88 & \bf 89.91 & 90.72 & \bf 88.13 & 89.79 & \bf 88.74 & \bf 88.98 & \bf 89.83 & \bf 84.86 \\
    \Xhline{3\arrayrulewidth}
\end{tabular}
}
\end{table*}

